Variable Extraction for Model Recovery in Scientific Literature

The global output of academic publications exceeds 5 million articles per year, making it difficult for humans to keep up with even a tiny fraction of scientific output. We need methods to navigate and interpret the artifacts -- texts, graphs, charts, code, models, and datasets -- that make up the literature. This paper evaluates various methods for extracting mathematical model variables from epidemiological studies, such as ``infection rate ($\alpha$),'' ``recovery rate ($\gamma$),'' and ``mortality rate ($\mu$).'' Variable extraction appears to be a basic task, but plays a pivotal role in recovering models from scientific literature. Once extracted, we can use these variables for automatic mathematical modeling, simulation, and replication of published results. We introduce a benchmark dataset comprising manually-annotated variable descriptions and variable values extracted from scientific papers. Based on this dataset, we present several baseline methods for variable extraction based on Large Language Models (LLMs) and rule-based information extraction systems. Our analysis shows that LLM-based solutions perform the best. Despite the incremental benefits of combining rule-based extraction outputs with LLMs, the leap in performance attributed to the transfer-learning and instruction-tuning capabilities of LLMs themselves is far more significant. This investigation demonstrates the potential of LLMs to enhance automatic comprehension of scientific artifacts and for automatic model recovery and simulation.

==> src/abstract.tex <==




% In the face of an overwhelming deluge of academic publications, with global output exceeding 5 million articles per year, the capacity of human scholars to digest, comprehend, and utilize this vast expanse of knowledge is significantly challenged. This saturation highlights the critical need for improved methods to navigate and interpret the myriad scientific artifacts—texts, graphs, charts, codes, models, and datasets—that make up this literature. Addressing this imperative, our study begins in the domain of epidemiology, evaluating the efficacy of various approaches to extract variables from the literature. Variable extraction, a seemingly basic yet fundamentally crucial task, plays a pivotal role in recovering models from scientific literature, facilitating a deeper understanding and application of research findings. \new{We introduce a manually-annotated dataset comprising \emph{variable descriptions} and \emph{variable values} extracted from scientific papers, which serves as a foundation for developing information extraction systems to support mathematical modeling and simulation. Based on this dataset, we present several baseline methods for variable extraction based on Large Language Models (LLMs) and rule-based information extraction systems. Our analysis shows that LLM-based solutions perform the best}. Despite the incremental benefits of combining \new{rule-based extraction} outputs with LLMs, the leap in performance attributed to the \new{transfer-learning and instruction-tunning} capabilities of LLMs themselves is far more significant. This investigation not only demonstrates the potential of LLMs to enhance the comprehension and utilization of scientific artifacts amidst the current flood of publications but also points towards a more efficient and accurate future for scientific research, particularly in the critical area of \new{mathematical} model recovery \new{and simulation}.

